Back-reaction of the Hawking radiation flux on a gravitationally collapsing star II

A star collapsing gravitationally into a black hole emits a flux of radiation, known as Hawking radiation. When the initial state of a quantum field on the background of the star, is placed in the Unruh vacuum in the far past, then in the exterior Hawking radiation corresponds to a flux of positive energy radiation travelling outwards from near the surface to future infinity. Based on pair creation, the evaporation of the collapsing star can be equivalently described by the absorption of an ingoing negative energy flux of radiation travelling towards the center of the star. Here, we are interested in the evolution of the star during its collapse. Thus we include the backreaction of the negative energy Hawking flux in the interior geometry of the collapsing star when writing the full 4-dimensional Einstein and hydrodynamic equations. Hawking radiation emitted before the star passes through its Schwarzschild radius slows down and reverses the collapse of the star. The star evaporates without forming an horizon or a singularity. This study provides a more realistic investigation than the one first presented in [1], since the backreaction of Hawking radiation flux on the collapsing star is studied in the case when the initial state of the field is in Unruh's vacuum.

==> Makefile <==
# Makefile for papers
PAPER = paper

# Figure variables
GPI_SCRIPTS := $(shell find . -name '*.gpi')
GPI_FIGURES  = $(GPI_SCRIPTS:makeplots-%.gpi=%.pdf)
XFIG_FILES  := $(shell find . -name '*.fig')
XFIGURES    = $(XFIG_FILES:%.fig=%.pdf)
SVG_FILES   := $(shell find . -name '*.svg')
SVG_FIGURES = $(SVG_FILES:%.svg=%.pdf)
AGR_FILES   := $(shell find . -name '*.agr')
AGR_FIGURES = $(AGR_FILES:%.agr=%.pdf)
PY_FILES   := $(shell find . -name 'q*.py')
PY_FIGURES  = $(PY_FILES:%.py=%.pdf)

MANUAL_FIGURES = $(shell find . -name  '*.png') \
#	Figures/Fig1.pdf Figures/Fig2.pdf 

AUTO_FIGURES := $(GPI_FIGURES) $(XFIGURES) $(SVG_FIGURES) $(AGR_FIGURES) \
	$(PY_FIGURES)

# Included tex files
TABLE_INCLUDES := $(shell find . -name 'Table*.tex')

svn:
	svn update
	make
git:
	git svn rebase
	make

.DEFAULT_GOAL := all
all: $(PAPER).pdf

.PHONY: figs
figs: $(AUTO_FIGURES)

# skip dvi and ps, as some figures are only availabe in pdf
$(PAPER).pdf: $(PAPER).tex $(AUTO_FIGURES) $(MANUAL_FIGURES) $(TABLE_INCLUDES)
	pdflatex -draftmode -file-line-error $<
#	bibtex $(PAPER)
#	pdflatex -draftmode -file-line-error $<
	pdflatex -file-line-error $<

# Automatically make pdf files from .gpi (gnuplot) scripts
%.pdf: makeplots-%.gpi
	gnuplot $<

# Automatically make pdf files from .fig files
%.pdf: %.fig
	fig2mpdf $<

# Automatically make pdf files from .svg files
%.pdf: %.svg
	inkscape -D -z --file=$< --export-pdf=$@

# Automatically make pdf files from .agr files
%.pdf:%.agr
	xmgrace -hardcopy -hdevice EPS -printfile epsfig.eps $<
	epstopdf --outfile=$@ epsfig.eps
	rm -f epsfig.eps

# Automatically make pdf files from .py files
%.pdf:%.py
	python $<

# The || : is there to make sure that subsequent lines get executed even if
# some of the removes fail because the files to be removed do not exist.
clean:
	@rm -f *.aux || :
	@rm -f *.dvi || :
	@rm -f *.out || :
	@rm -f *Notes.bib || :
	@rm -f *.log || :
	@rm -f *.bbl || :
	@rm -f *.blg || :
	@rm -f *.backup || :
	@rm -f *~ || :
	@rm -f $(AUTO_FIGURES) || :
	@rm -f $(PAPER).pdf || :


